An Algebraic Approach to Learning and Grounding

We consider the problem of learning the semantics of composite algebraic expressions from examples. The outcome is a versatile framework for studying learning tasks that can be put into the following abstract form: The input is a partial algebra $\alg$ and a finite set of examples $(\varphi_1, O_1), (\varphi_2, O_2), \ldots$, each consisting of an algebraic term $\varphi_i$ and a set of objects~$O_i$. The objective is to simultaneously fill in the missing algebraic operations in $\alg$ and ground the variables of every $\varphi_i$ in $O_i$, so that the combined value of the terms is optimised. We demonstrate the applicability of this framework through case studies in grammatical inference, picture-language learning, and the grounding of logic scene descriptions.

==> triangle.tex <==

\begin{figure}[tb]
\begin{tikzpicture}[node distance=15mm, auto]

% The angles of x,y,z-axes
\newcommand\xaxis{210}
\newcommand\yaxis{-30}
\newcommand\zaxis{90}

  \newcommand\nt[4]{
	\begin{scope}[shift={(#1,#2)},rotate=#3,scale=#4]
	\node[transform shape, fill=lightblue!50, rectangle, draw, very thick,inner sep=5pt] (mid) {$S$};
	\end{scope}
  }

  \newcommand\nte[4]{
	\begin{scope}[shift={(#1,#2)},rotate=#3,scale=#4]
	\node[transform shape, fill=lightblue!50, rectangle, draw, very thick,inner sep=5pt] (mid) {$A$};
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, above = 10pt of mid] (top) {};
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, below left = 7pt of mid] (left) {};
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, below right = 7pt of mid] (right) {};
		\draw [very thick] (mid)--(top);
		\draw [very thick] (mid)--(left);
		\draw [very thick] (mid)--(right);
	\end{scope}
  }

	% First rule
	\nt{0}{2}{0}{1};
	\node (n) at (1,2){\Large $\rightarrow$} ;
	\nte{2}{2}{0}{1};

	% Second rule
	\begin{scope}[shift={(4.5,0)},rotate=0]
	\nte{0.2}{2}{0}{1};

	\node (n) at (1.5,2){\Large $\rightarrow$};

	\nte{3.0}{2.5}{0}{0.8};
	\nte{2.35}{1.38}{120}{0.8};
	\nte{3.65}{1.38}{240}{0.8};
	\end{scope}

	% Third rule
	\begin{scope}[shift={(10.5,0)},rotate=0]
	\nte{0.2}{2}{0}{1};

	\node (n) at (1.5,2){\Large $\rightarrow$};

	\node[transform shape] (dmid) at (3,2){} ;
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, below = 3pt of dmid] (dtop) {};
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, above left = 12pt of dmid] (dleft) {};
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, above right = 12pt of dmid] (dright) {};

	\draw [very thick] (dtop)--(dleft);
	\draw [very thick] (dleft)--(dright);
	\draw [very thick] (dright)--(dtop);
	\end{scope}

\end{tikzpicture}

\vspace{5pt}
\begin{tikzpicture}[node distance=15mm, auto]

% The angles of x,y,z-axes
\newcommand\xaxis{210}
\newcommand\yaxis{-30}
\newcommand\zaxis{90}

  \newcommand\nt[4]{
	\begin{scope}[shift={(#1,#2)},rotate=#3,scale=#4]
	\node[transform shape, rectangle, fill=lightblue!50, draw, very thick,inner sep=5pt] (mid) {$S$};
	\end{scope}
  }

  \newcommand\nte[4]{
	\begin{scope}[shift={(#1,#2)},rotate=#3,scale=#4]
	\node[transform shape, rectangle, fill=lightblue!50, draw, very thick,inner sep=5pt] (mid) {$A$};
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, above = 10pt of mid] (top) {};
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, below left = 7pt of mid] (left) {};
	\node[transform shape, draw, ultra thick,circle,inner sep=1.5pt, fill=black, below right = 7pt of mid] (right) {};
		\draw [very thick] (mid)--(top);
		\draw [very thick] (mid)--(left);
		\draw [very thick] (mid)--(right);
	\end{scope}
  }

	\begin{scope} [scale=0.65]

	% First rule
	\nt{0}{2}{0}{1};
	\node (n) at (1.25,2){\Large $\Rightarrow$} ;
	\nte{2.75}{2}{0}{1};
	\node (m) at (4.3,2){\Large $\Rightarrow$} ;

	\begin{scope}[shift={(3.2,0)},rotate=0]
	\nte{3.0}{2.5}{0}{0.8};
	\nte{2.35}{1.38}{120}{0.8};
	\nte{3.65}{1.38}{240}{0.8};
	\end{scope}
	
	\node (o) at (8.3,2){\Large $\Rightarrow$} ;

	\begin{scope}[shift={(8.5,1.45)},rotate=0,scale=0.7]
	\nte{3.0}{2.5}{0}{0.8};
	\nte{2.35}{1.38}{120}{0.8};
	\nte{3.65}{1.38}{240}{0.8};
	\end{scope}

	\begin{scope}[shift={(7.65,0)},rotate=0,scale=0.7]
	\nte{3.0}{2.5}{0}{0.8};
	\nte{2.35}{1.38}{120}{0.8};
	\nte{3.65}{1.38}{240}{0.8};
	\end{scope}

	\begin{scope}[shift={(9.35,0)},rotate=0,scale=0.7]
	\nte{3.0}{2.5}{0}{0.8};
	\nte{2.35}{1.38}{120}{0.8};
	\nte{3.65}{1.38}{240}{0.8};
	\end{scope}
	
	\node (p) at (14.8,2){\Large $\Rightarrow$ \, ... \, $\Rightarrow$} ;
	\end{scope}

        \node[inner sep=0pt] (russell) at (13.0,1.2)
            {\includegraphics[width=.25\textwidth]{sierpinski.png}};

	\end{tikzpicture}

%\includegraphics[bb= 50 500 600 680,width=\textwidth]{HRG.pdf}
	\caption{ Top row: Three productions in an HRG $G$ with nonterminals $S$ and $A$ (drawn in blue). The productions rewrite nonterminals into graphs consisting of nonterminals, as well as of terminal edges and nodes (drawn in black). Bottom row: a sample derivation in $G$ that produces a graph with the same topology as (a finite approximation of) the Sierpinski triangle.}
\label{fig:HRG}
\end{figure}
